The Fusion of Large Language Models and Formal Methods for Trustworthy AI Agents: A Roadmap

Large Language Models (LLMs) have emerged as a transformative AI paradigm, profoundly influencing daily life through their exceptional language understanding and contextual generation capabilities. Despite their remarkable performance, LLMs face a critical challenge: the propensity to produce unreliable outputs due to the inherent limitations of their learning-based nature. Formal methods (FMs), on the other hand, are a well-established computation paradigm that provides mathematically rigorous techniques for modeling, specifying, and verifying the correctness of systems. FMs have been extensively applied in mission-critical software engineering, embedded systems, and cybersecurity. However, the primary challenge impeding the deployment of FMs in real-world settings lies in their steep learning curves, the absence of user-friendly interfaces, and issues with efficiency and adaptability. This position paper outlines a roadmap for advancing the next generation of trustworthy AI systems by leveraging the mutual enhancement of LLMs and FMs. First, we illustrate how FMs, including reasoning and certification techniques, can help LLMs generate more reliable and formally certified outputs. Subsequently, we highlight how the advanced learning capabilities and adaptability of LLMs can significantly enhance the usability, efficiency, and scalability of existing FM tools. Finally, we show that unifying these two computation paradigms -- integrating the flexibility and intelligence of LLMs with the rigorous reasoning abilities of FMs -- has transformative potential for the development of trustworthy AI software systems. We acknowledge that this integration has the potential to enhance both the trustworthiness and efficiency of software engineering practices while fostering the development of intelligent FM tools capable of addressing complex yet real-world challenges.

==> eval.tex <==
\section{Evaluation}

This section discusses brief/preliminary evaluation results on the agents and analyses which agent is suited for what use cases.

==> xinyue_yifan/PATAgent_old.tex <==
% \subsubsection{Overall Framework}
\noindent\textbf{Motivation}
% \subsubsection{PAT Agent} 
PAT Agent is designed to take advantage of the strengths of LLMs and PAT to counter their respective weaknesses. A major limitation of LLMs is their tendency to produce content that seems plausible but contains logical errors, a problem referred to as hallucination~\cite{ji2023survey}. This becomes especially risky when LLMs are deployed in safety-critical domains~\cite{yao2023llm}. In contrast, formal verification tools like PAT provide mathematical assurances of system correctness, though their complexity and steep learning curve make them difficult for non-experts to use, unlike LLMs, which are more user-friendly. This presents a challenge in balancing ease of use with reliability, particularly for general users.

PAT Agent bridges this gap by combining the advantages of LLMs with formal verification tools. LLMs are recognized for their ease of use, enabling non-technical users to interact through natural language. PAT Agent leverages this capability by accepting a system description in natural language from the user, generating corresponding processes using an LLM, and refining them iteratively based on feedback from PAT. This refinement is facilitated by an Automated Prompt Engineer (APE)~\cite{cheng2023black,zhou2022large}, which optimizes the interaction between the LLM and PAT.

The aim of PAT Agent is not only to facilitate users to generate syntactically correct code or system constructs, but also to guarantee that these outputs comply with logical properties and pass formal verification, thus enhancing the reliability of content produced by LLMs.

\subsubsection{Overview}
The overall workflow for building verification agents should include the following steps:

\begin{enumerate}[leftmargin=*] 
\item \textbf{Natural Language Input:}
Users provide a description of a system in natural language, specifying desired behaviors or properties. For instance, they might describe a mutual exclusion protocol or outline expected system behaviors.

\item \textbf{LLM Planning:}
An LLM with strong reasoning capabilities translates the natural language input into a detailed, structured plan. This plan breaks down the system description into specific instructions, including a one-to-one mapping of logical steps, such as defining variables, specifying state transitions, and drafting preliminary assertions.

\item \textbf{LLM Code (Assertion) Completion:}
Following the structured plan, a specialized LLM trained in syntax and logic generates the code and assertions required to implement the system. This generation is treated as a completion task, where the model fills in the details based on the planning phase rather than creating the code from scratch. The structured approach enhances precision and reduces the likelihood of errors in the generated outputs.

\item \textbf{Formal Verification:}
The generated code and assertions are submitted to a formal verification tool. This tool evaluates the artifacts to ensure they comply with the logical properties and behaviors specified in the initial input. 
% Any detected violations, inconsistencies, or failed assertions are flagged and documented for further refinement.

\item \textbf{Feedback Generation:}
Feedback from the formal verification tool highlights issues such as syntax errors or logical inconsistencies. This feedback is processed by an Automated Prompt Engineer (APE), which refines the LLM's prompts and provides updated instructions.

\item \textbf{Iterative Improvement:}
The LLM iteratively refines the code and assertions based on feedback until all formal verification checks are successfully passed. Through this iterative process, the framework ensures that the final system model is logically sound, adheres to the desired specifications, and is ready for deployment.

    % \item Natural Language Input: Users provide a description of the system in natural language (e.g., a mutual exclusion protocol or system behavior).
    
    % \item Assertion Generation and Refinement: The LLM generates assertions (i.e., system properties that must be satisfied) based on the user input. These assertions undergo an iterative refinement process to ensure their validity and completeness, accurately representing the required system conditions. Once confirmed as correct, the process proceeds to code generation.
    
    % \item LLM Code Generation: After the assertions are validated, the LLM produces formal code that conforms to PAT’s syntax and logical structure, designed to meet the refined assertions.
\end{enumerate}


In the following part, we will illustrate our verification agent framework based on a well-used verification tool, PAT, and show specifically how to interactively leverage the features of FM and LLM to facilitate such a PAT agent.
% \subsubsection{Other Verification Agents}

However, we acknowledge that such an agent framework is highly generalizable and can be adapted for tools like Alloy, Prism, B Method, Isabelle, and HOL. Its modular design enables the Planning LLM to learn tool-specific semantics and the Code Generation LLM to produce corresponding formal code and assertions. By tailoring feedback and refinement loops for each tool, the framework seamlessly integrates LLM-driven development with diverse formal verification processes.

% introduce the PAT Agent, an integration of a large language model (LLM) with a formal verification tool (PAT: Process Analysis Toolkit~\cite{sun2008model}). 

\subsubsection{PAT}

% A PAT Agent utilizes PAT to actively improve the quality and guarantee the correctness of LLM-generated content. It introduces an automatic interaction between LLMs and PAT to iteratively refine LLM-generated code, ensuring that the outputs meet formal verification standards.

\noindent\textbf{Motivation}
% \subsubsection{PAT Agent} 
PAT Agent is designed to take advantage of the strengths of LLMs and PAT to counter their respective weaknesses. A major limitation of LLMs is their tendency to produce content that seems plausible but contains logical errors, a problem referred to as hallucination~\cite{ji2023survey}. This becomes especially risky when LLMs are deployed in safety-critical domains~\cite{yao2023llm}. In contrast, formal verification tools like PAT provide mathematical assurances of system correctness, though their complexity and steep learning curve make them difficult for non-experts to use, unlike LLMs, which are more user-friendly. This presents a challenge in balancing ease of use with reliability, particularly for general users.

PAT Agent bridges this gap by combining the advantages of LLMs with formal verification tools. LLMs are recognized for their ease of use, enabling non-technical users to interact through natural language. PAT Agent leverages this capability by accepting a system description in natural language from the user, generating corresponding processes using an LLM, and refining them iteratively based on feedback from PAT. This refinement is facilitated by an Automated Prompt Engineer (APE)~\cite{cheng2023black,zhou2022large}, which optimizes the interaction between the LLM and PAT.

The aim of PAT Agent is not only to facilitate users to generate syntactically correct code or system constructs, but also to guarantee that these outputs comply with logical properties and pass formal verification, thus enhancing the reliability of content produced by LLMs.

\noindent\textbf{Motivating Example.}
In the development of a car system, ensuring that the key is never locked inside the car is a critical requirement. This safeguard is essential for user convenience and safety, as locking the key inside could result in costly locksmith services, delays, or emergencies in dangerous areas. The system must ensure logical consistency in different operations to avoid such consequences.

% $[key == i \&\& owner[i] == near]leavekey{key = incar;}$

We begin by asking an LLM (gpt-4o-2024-08-06) to directly generate the system code based on a high-level description. While the LLM has learned syntax rules and demonstrates effective planning capabilities, the generated implementation contains a critical logical flaw: it allows the key to be locked inside the car. This issue arises due to a hallucination by GPT-4o, which incorrectly assumes that placing the key into a currently locked car is a valid scenario, contradicting commonsense reasoning. 
\vspace{-8pt}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize, showlines=false]
[key == i && owner[i] == near]leavekey{key = incar;}
\end{lstlisting}
\vspace{-8pt}

Consequently, the resulting system design deviates from the intended behavior, compromising its reliability and safety.

% Besides, the current logic also defines an ambiguous requirement for locking the door: the door can only be locked when it is unlocked, the owner is near, and the key is not inside.
% \vspace{-6pt}
% \begin{lstlisting}[basicstyle=\ttfamily\footnotesize, showlines=false]
% [door == unlock && owner[i] == near && key != incar]
% lockdoor.i{door = lock;}
% \end{lstlisting}
% \vspace{-6pt}

To address this issue, we use PAT to formally verify the generated system. PAT identifies an error trace (i.e., a sequence of operations) that leads to the key being locked inside the car, providing feedback that highlights flaws in the logic governing key and door operations. By analyzing this error trace, the LLM identifies the aforementioned logical flaw and corrects it by imposing stricter restrictions on when the key can be left inside the car. Additionally, it establishes clear conditions for locking the door, ensuring alignment with the intended system behavior.

\vspace{-6pt}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize, showlines=false]
[key == i && owner[i] == near && door == open]
leavekey{key = incar;}
\end{lstlisting}
\vspace{-6pt}

\vspace{-6pt}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize, showlines=false]
[(owner[i] == near && key == i) || owner[i] == in]
lockdoor.i{door = lock;}
\end{lstlisting}
\vspace{-6pt}

The refined implementation, guided by PAT feedback, results in a system that can now be formally verified to ensure the key will never be locked inside the car. This example highlights the powerful synergy between formal verification and LLM-driven development. LLMs ease the process of system development, while tools like PAT provide rigorous guarantees by identifying and rectifying logical inconsistencies. Together, they create a robust and user-friendly approach to formal system development, ensuring critical requirements are met with precision.

% \com{which example is more reasonable: lock door then put the key inside? or can lock the door when the key is inside?}



\noindent\textbf{Prototype}

To implement the PAT Agent, we build it on the LangChain pipeline, leveraging its streamlined implementation and modularized memory system to efficiently manage intermediate states and iterative refinements during formal verification. This allows seamless integration of LLM capabilities with formal verification tools. We illustrate the prototype in Figure~\ref{fig:prototype}.

\begin{figure}[h]
 \begin{centering}
  \includegraphics[width=1\linewidth]{xinyue&yifan/PAT_Agent_Prototype.png}
  \par\end{centering}
 \caption{PAT Agent Prototype.}
 \label{fig:prototype}
\end{figure}



==> yufan/SMT_Solver_old.tex <==
\subsection{Faithful LLMs with SMT Solvers}
Satisfiability Modulo Theories (SMT) solvers are tools designed to determine the satisfiability of logical formulas across various theories, such as arithmetic, bit-vectors, and arrays. They play a crucial role in formal verification, program analysis, and automated reasoning. 
% Integrating SMT solvers with LLMs has shown promise in enhancing logical reasoning and code analysis tasks.
% \subsubsection{Integrating SMT Solvers with LLMs}
% \paragraph{Existing Solutions.}
Recent studies~\cite{deng2024enhancing,pan2023logic,wang2024dataflow,ye2024satlm} have investigated the integration of SMT solvers to enhance the accuracy and reliability of LLMs for logic reasoning.% Specifically, these works leverage LLMs to synthesize specification code that outsources delicate reasoning to external expert tools, given the specific

% For example, \cite{wang2024pythonsymbolicexecutionllmpowered} developed LLM-Sym, an LLM -agent that automatically invokes Z3, a widely used of the most popular SMT Solver developedsigned by Microsoft Research, towhen solve ing execution path constraints in Python programs,.

% For example,  \cite{deng2024enhancing} proposed an approach that combines LLMs with the Z3 solver and a Self-Refinement Module to address logical reasoning tasks. 

% on improving the logical reasoning capabilities of Large Language Models (LLMs) by integrating them with a Z3 symbolic solver and incorporating a Self-Refinement Module. It evaluates the integration of LLMs with a Z3 symbolic solver to solve various reasoning tasks. Results showed accuracy improvements of 4.86\% with GPT-3.5-Turbo and 7.82\% with GPT-4 compared to the baseline Logic-LM on four datasets.

\paragraph{Technical Challenges.}
% verbose constraints, no correctness guarantees, syntax error
While LLMs can generate logical constraints or assist in translating natural language into SMT formulas, they may generate suboptimal or overly verbose constraints that further burden the solver. 
Besides,
LLMs lack guarantees of correctness or logical consistency in their outputs. They may introduce subtle inaccuracies or ambiguities when generating SMT constraints, leading to invalid results or harder-to-interpret solutions.
On the other hand, LLMs often lack domain-specific knowledge or fail to align outputs with the precise formal syntax required by SMT solvers. They may also generate semantically correct but syntactically invalid formulas, which solvers cannot process.

\paragraph{Our Insights.} 
(1) Multiple LLMs Debating: Involves multiple LLMs working collaboratively or adversarially to critique, validate, and refine each other's outputs.
The system can combine multiple LLMs to generate SMT code from Natural Language input.
Other LLMs act as "critics," analyzing the generated SMT code for logical consistency, syntactic correctness, and adherence to the problem's description, which can reduce natural language ambiguity.
Critics can challenge the code by asking clarifying questions or suggesting alternative formulations.

(2) Test Generation: Automatically create test cases to validate the correctness and performance of the SMT code against expected behavior.
The system can use fuzzing for test case generation by applying LLMs to create adversarial inputs and ensure that the generated SMT code is produced correctly.
It can also mutate the variants in the SMT code and the natural language description and then use two LLMs to compare the solutions to check the consistency of the natural language description and the SMT code.

(3) Self-Correction: Leverage feedback from tests, critics, or the solver itself to iteratively refine the SMT code.
The system identifies errors from solver feedback, categorizing them as syntax issues (e.g., invalid SMT-LIB syntax), semantic misalignments (e.g., logical inconsistencies or mismatches between the natural language and SMT code), or performance bottlenecks (e.g., slow or incomplete solver responses). Based on these insights, the system employs an LLM to debug and regenerate problematic sections of code, ensuring improvements are targeted and context-aware. This iterative refinement process, combined with validation through re-testing, ensures the SMT code converges toward correctness and efficiency.

\subsubsection{Case Study}

To illustrate our perspective, we give our recent exploration of the interaction between LLMs and Z3, a widely used satisfiability modulo theories (SMT) solver developed by Microsoft Research. 
Z3 accepts inputs in the form of a simple-sorted formula expressed in first-order logic (FOL), which may contain symbols with predefined meanings as defined by various underlying theories. These theories encompass domains such as arithmetic, bit-vectors, arrays, etc., making Z3 particularly well-suited for reasoning about a wide range of logical constraints. 

Consider a scenario where the user asks the LLM agent to solve a scheduling problem: 

\textit{"Can you help plan a meeting for a team of three people—David, Emma, and Sarah? David is free on Monday or Tuesday, Emma is free on Tuesday or Wednesday, and Sarah is free only on Monday or Wednesday. Find a common day when all three are available."}

The integration of the Z3 solver with the LLM agent follows a pipeline that includes:
\paragraph{Natural Language Understanding:} 
The LLM agent analyzes the query to understand:
There are three participants: David, Emma, and Alex.
Each participant has specific availability constraints:
David: Monday or Tuesday.
Emma: Tuesday or Wednesday.
Alex: Tuesday or Thursday. 
Find a common day when all four (David, Emma, and Alex) are available.

\paragraph{Formalization of Constraints:} The agent translates the natural language constraints into a formal representation suitable for Z3:
\begin{minted}[linenos]{python}
# Define days of the week
days = ["Monday", "Tuesday", "Wednesday", "Thursday"]
David_free = [Bool(f"David_free_{day}") for day in days]
Emma_free = [Bool(f"Emma_free_{day}") for day in days]
Alex_free = [Bool(f"Alex_free_{day}") for day in days]
# Create a solver
solver = Solver()
# Define constraints for each person's availability
solver.add(Or(David_free[0], David_free[1])) 
solver.add(Or(Emma_free[1], Emma_free[2]))  
solver.add(Or(Alex_free[1], Alex_free[3]))   
# Add constraints that ensure a common day for all three
common_day_constraints = [And(David_free[i], 
Emma_free[i], Alex_free[i]) for i in range(len(days))]
solver.add(Or(common_day_constraints)) 
\end{minted}

\paragraph{Self-Correction:}
If the initial translation has issues (e.g., missing constraints or logical errors), the agent can identify and correct them.

\begin{minted}[linenos]{python}
# Constraints for David
solver.add(David_free[0] == True) 
solver.add(David_free[1] == True) 
solver.add(And(Not(David_free[2]), Not(David_free[3]))) 
# Constraints for Emma
solver.add(Emma_free[1] == True)  
solver.add(Emma_free[2] == True)  
solver.add(And(Not(Emma_free[0]), Not(Emma_free[3])))  
# Constraints for Alex
solver.add(Alex_free[1] == True)  
solver.add(Alex_free[3] == True) 
solver.add(And(Not(Alex_free[0]), Not(Alex_free[2])))  
\end{minted}

\paragraph{Test Generation:}
The agent mutates the constraints and involves tweaking the availability for each individual to create new conditions.
Mutated Constraints:
David: Free on Monday and Wednesday.
Emma: Free on Tuesday and Thursday.
Alex: Free on Monday and Thursday.
The updated Z3 code is as follows:
\begin{minted}[linenos]{python}
# Mutated constraints for David
solver.add(And(David_free[0], David_free[2])) 
solver.add(And(Not(David_free[1]), Not(David_free[3]))) 
# Mutated constraints for Emma
solver.add(And(Emma_free[1], Emma_free[3]))  
solver.add(And(Not(Emma_free[0]), Not(Emma_free[2]))) 
# Mutated constraints for Alex
solver.add(And(Alex_free[0], Alex_free[3])) 
solver.add(And(Not(Alex_free[1]), Not(Alex_free[2]))) 
\end{minted}

\paragraph{Problem Solving:} The translated constraints are fed into the Z3 solver, which checks the satisfiability of the formula and computes a solution if possible.
\begin{minted}[linenos]{python}
# Check for a solution
if solver.check() == sat:
    model = solver.model()
    common_days = [days[i] for i in range(len(days)) 
    if model.evaluate(David_free[i]) 
       and model.evaluate(Emma_free[i]) 
       and model.evaluate(Alex_free[i])]
    print(f"Common day(s) when everyone is free:
    {common_days}")
else:
    print("No common day when everyone is free.")
\end{minted}

\paragraph{Multiple LLM Debating:}
LLM A: Generates the initial constraints.
LLM B: Critiques the constraints, identifying potential issues such as missing exclusivity rules or improperly translated logic.
LLM C: Suggests refinements, such as introducing mutual exclusivity or expanding constraints to handle edge cases.
Consensus: The output with the highest confidence score (e.g., most accurate or simplest) is selected for testing and execution.

\paragraph{Solution Interpretation:} The LLM agent receives the solution from the Z3 solver and translates it back into natural language for the user.
The only day when all three are free is Tuesday. The output should be: Common day(s) when everyone is free: ['Tuesday'].

This example demonstrates how the LLM agent leverages the power of formal verification tools like Z3 to perform logical reasoning and constraint-solving in a user-friendly manner.
Integrating Z3 with an LLM agent opens up new possibilities for combining natural language understanding with formal methods. 
We make formal methods more accessible by enabling users to pose complex, constraint-based problems in natural language and having the system automatically solve them using formal logic. 
Future research could focus on improving the natural language translation process, enabling the agent to handle more complex problems, and integrating other solvers for specialized domains.
